Photons in a Ball

The electromagnetic field inside a spherical cavity of large radius R is considered in the presence of stationary charge and current densities. R provides infra-red regularization while maintaining gauge invariance. The quantum ground state of physical photons forming the magnetic field is found to be a coherent state with a definite mean occupation number. The electric field, which is determined by the Gauss law constraint, is maintained by a minimum uncertainty coherent state, according to the projection operator approach to the quantization of constrained systems. The mean occupation number of this state is proportional to the square of the total charge. The results confirm formulae obtained previously from a calculation with a finite photon mass for infra-red regularization.

==> em3.tex <==
\section{Quantization of em field in radial gauge}
\label{em}
\subsection{Canonical pairs of variables}

Consider the Lagrangian for an electromagnetic field living inside a sphere of radius $R$,
%
\begin{equation}
\label{em:lag}
	\Lag = -\frac14 F_{\mu\nu} F^{\mu\nu} - \frac1{2\alpha} (n^\mu A_\mu)^2 - j^\mu A_\mu~,
\end{equation}
%
where $F_{\mu\nu}=\partial_\mu A_\nu - \partial_\nu A_\mu$ is the field strength, $j^\mu$ is a conserved current, the four-vector in the gauge term is
%
\begin{equation}
\label{em:n.def}
	n^\mu = \left(1,\bn\right) \qquad \text{with}\quad \bn =\frac1R \br~,
\end{equation}
%
and $\alpha$ is a parameter of dimension $L^2$. With the choice \eqref{em:n.def}, $n^\mu$ is light-like inside the sphere and becomes null on the boundary. 

The canonical momenta, which formally satisfy the Poisson brackets
%
\begin{equation}
\label{em:poisson}
	\pois{A_\mu(\bx)}{\pi^\nu(\by)} = \delta_\mu^\nu\, \delta^3(\bx-\by)~,
\end{equation}
%
are 
%
\begin{equation}
\label{em:momenta}
	\pi^0 = 0~,\qquad \pi^i =F^{i0}~.
\end{equation}
%
The Hamiltonian is found to be
%
\begin{equation}
\label{em:ham}
	H = \int \rmd^3 r\left[ \frac12 \pi^i \pi^i + \frac14 F_{ij}F^{ij} - \partial_i \pi^i A_0 
	+\frac1{2\alpha} (n^\mu A_\mu)^2 +j^\mu A_\mu \right]~,
\end{equation}
%
where a total derivative has been dropped by setting $A_0$ to zero on the surface of the sphere. 

Before constructing the constraint algebra we decompose all variables in the spherically harmonic eigenfunctions of the Laplacian on the sphere, as summarized in appendix~\ref{app:expansion}. It turns out to be useful to define the combinations
%
\begin{subequations}
\label{em:new.modes}
\begin{align}
	\hat{A}_{lmk} &= \sqrt{\frac{l}{2l+1}} A^{(1)}_{lmk} - \sqrt{\frac{l+1}{2l+1}} A^{(2)}_{lmk}~,\\
	\tilde{A}_{lmk} &= \sqrt{\frac{l+1}{2l+1}} A^{(1)}_{lmk} + \sqrt{\frac{l}{2l+1}} A^{(2)}_{lmk}~,
\end{align}
\end{subequations}
%
and analogously for the momenta $\pi^i$ and the current $j^i$. After some calculation, one obtains for the Hamiltonian \eqref{em:ham}
%
\begin{equation}
\label{em:ham2}
\begin{aligned}
	H &= \sum_{lmk}\Bigg\{ 
	 	\frac12 \left( |\hat{\pi}_{lmk}|^2 + |\tilde{\pi}_{lmk}|^2 + |\pi^{(3)}_{lmk}|^2 \right) 
		+\frac12 k^2 \left(|\hat{A}_{lmk}|^2+ |A^{(3)}_{lmk}|^2 \right) 
		+k \re\left( A^{(0)}_{lmk} \tilde{\pi}^\ast_{lmk} \right)\\
		&\quad +\frac1{2\alpha} \left| A^{(0)}_{lmk} -\frac{\sqrt{l(l+1)}}{kR} \hat{A}_{lmk} \right|^2
		+\frac1{2\alpha} \sum_{k'} \frac1{kk'R^2} \tilde{B}^{(l)}_{kk'} 
		\re \left(\tilde{A}_{lmk}\tilde{A}^\ast_{lmk'}\right)\\
		&\quad + \frac1{2\alpha} \sum_{k'}	\frac2{k'R} B^{(l)}_{kk'} 
		\re\left[\left(A^{(0)}_{lmk} -\frac{\sqrt{l(l+1)}}{kR} \hat{A}_{lmk}\right) \tilde{A}^\ast_{lmk'} \right]\\
		&\quad +\re\left( A^{(0)}_{lmk} j^{(0)\ast}_{lmk} + \hat{A}_{lmk} \hat{j}^\ast_{lmk}
		+ \tilde{A}_{lmk} \tilde{j}^\ast_{lmk} + A^{(3)}_{lmk} j^{(3)\ast}_{lmk} \right) \Bigg\}~,
\end{aligned}
\end{equation}
%
where the matrices $B^{(l)}_{kk'}$ and $\tilde{B}^{(l)}_{kk'}$ are defined by the integrals
%
\begin{align}
\label{em:Bmat.def}
	B^{(l)}_{kk'} &= \frac1{c^{(0)}_{lk}c^{(0)}_{lk'}} \int\limits_0^R \rmd r\, r^3 j_l(kr) \partial_r j_l(k'r)~,\\
\label{em:Bmat.tilde.def}
	\tilde{B}^{(l)}_{kk'} &= \frac1{c^{(0)}_{lk}c^{(0)}_{lk'}} 
	\int\limits_0^R \rmd r\, r^4 [\partial_r j_l(kr)][\partial_r j_l(k'r)]~,
\end{align}
%
respectively. We emphasize that the choice $\bn=\br/R$ is crucial for obtaining these expressions. 
Integrating by parts the integral in \eqref{em:Bmat.def}, one finds 
% 
\begin{equation}
\label{em:Bmat.prop}
	B^{(l)}_{kk'} =-\frac32 \delta_{kk'} + B^{(l)}_{[kk']}~, 
\end{equation}
%
where the brackets around the indices indicate the anti-symmetric part of the matrix.
Moreover, by completeness of the spherical Bessel functions, they satisfy the useful relation
%
\begin{equation}
\label{em:Bmat.rel}
	\sum_{k''} B^{(l)}_{k''k} B^{(l)}_{k''k'} = \tilde{B}^{(l)}_{kk'}~. 
\end{equation}
%
By virtue of this, the second and third lines of \eqref{em:ham2} can be combined into 
%
\begin{equation}
\label{em:ham.terms}
	\frac1{2\alpha} \left| A^{(0)}_{lmk} -\frac{\sqrt{l(l+1)}}{kR} \hat{A}_{lmk}  
	+\sum_{k'} \frac1{k'R} B^{(l)}_{kk'} \tilde{A}_{lmk'} \right|^2~.
\end{equation}


We are now ready to find the algebra of constraints and construct the Dirac brackets.
The first of \eqref{em:momenta} is a primary constraint, which in modes reads
% 
\begin{equation}
\label{em:constraint1}
	\phi^{(1)}_{lmk} = \pi^{(0)}_{lmk} \approx 0~.
\end{equation}
%
Invariance under time evolution leads to the secondary constraint
%
\begin{equation}
\label{em:constraint2}
	\phi^{(2)}_{lmk} 
	= k\tilde{\pi}_{lmk} +\frac1{\alpha} \left(A^{(0)}_{lmk} -\frac{\sqrt{l(l+1)}}{kR} \hat{A}_{lmk} 
	+\sum_{k'} \frac1{k'R} B^{(l)}_{kk'} \tilde{A}_{lmk'}\right) +j^{(0)}_{lmk} \approx 0~.
\end{equation}
%
Here, we recognize the combination appearing in \eqref{em:ham.terms}. 
The two constraints satisfy the algebra 
%
\begin{equation}
\label{em:constraint.algebra}
	\pois{\phi^{(a)}_{lmk}}{\phi^{(b)\ast}_{l'm'k'}} =C^{ab}_{lmk,l'm'k'}
	= \frac1\alpha \delta_{ll'}\delta_{mm'} 
	\begin{pmatrix} 0 & -\delta_{kk'} \\
	\delta_{kk'} & \frac2{R} B^{(l)}_{[kk']} \end{pmatrix}~.
\end{equation}
%
Hence, the inverse of the matrix \eqref{em:constraint.algebra} is 
%
\begin{equation}
\label{em:constraint.algebra.inverse}
	\left(C^{-1}\right)^{ab}_{lmk,l'm'k'}
	= \alpha \delta_{ll'}\delta_{mm'} 
	\begin{pmatrix} \frac2{R} B^{(l)}_{[kk']} & \delta_{kk'} \\
	-\delta_{kk'} & 0 \end{pmatrix}~.
\end{equation}
%
The next step is the construction of the Dirac brackets,
%
\begin{equation}
\label{em:dirac.def}
	\dirac{F}{G} = \pois{F}{G} - \pois{F}{\phi^{(a)\ast}} (C^{-1})^{ab} \pois{\phi^{(b)}}{G}~,
\end{equation}
%
where the summation over all indices is implied. The resulting non-vanishing Dirac brackets are
%
\begin{equation}
\label{em:dirac.brackets1}
	\dirac{\hat{A}_{lmk}}{\hat{\pi}^\ast_{l'm'k'}} = \dirac{\tilde{A}_{lmk}}{\tilde{\pi}^\ast_{l'm'k'}}
	= \dirac{A^{(3)}_{lmk}}{\pi^{(3)\ast}_{l'm'k'}} = \delta_{ll'} \delta_{mm'} \delta_{kk'}~,
\end{equation}
and
\begin{equation}
\label{em:dirac.brackets2}
\begin{aligned}
	\dirac{A^{(0)}_{lmk}}{\tilde{\pi}^\ast_{l'm'k'}} &= -\frac1{k'R}\, \delta_{ll'}\delta_{mm'} B^{(l)}_{kk'}~,\\
	\dirac{A^{(0)}_{lmk}}{\hat{\pi}^\ast_{l'm'k'}} &= \frac1{kR} \sqrt{l(l+1)}\, \delta_{ll'} \delta_{mm'} \delta_{kk'}~,\\
	\dirac{A^{(0)}_{lmk}}{\tilde{A}^\ast_{l'm'k'}} &= \alpha k\,  \delta_{ll'} \delta_{mm'} \delta_{kk'}~,\\
	\dirac{A^{(0)}_{lmk}}{A^{(0)\ast}_{l'm'k'}} &= \frac{2\alpha}{R}\, \delta_{ll'} \delta_{mm'} B^{(l)}_{[kk']}~.
\end{aligned}
\end{equation}








\subsection{Imposing the constraint}

We shall now study the constraint \eqref{em:constraint2} in more detail. Let us start by decomposing the variables in  \eqref{em:constraint2} according to the formulas in appendix~\ref{app:expansion}. After using the properties of the vector spherical harmonics and the recurrence formulas for spherical Bessel functions, one obtains
%
\begin{equation}
\label{em:const.dec}
	\sum\limits_{lmk} \frac{Y_{lm}(\Omega)}{c^{(0)}_{lk}} \left\{ j_l(kr) \left[ k\tilde{\pi}_{lmk} + j^{(0)}_{lmk} 
	+\frac1{\alpha} A^{(0)}_{lmk} -\frac{\sqrt{l(l+1)}}{\alpha k R} \hat{A}_{lmk} \right] 
	+ \frac{r}{\alpha k R} \partial_r j_l(kr) \tilde{A}_{lmk} \right\} =0~.
\end{equation}
%
As before, the choice $\bn =\br/R$ is crucial in the terms with $\hat{A}$ and $\tilde{A}$. Then, using \eqref{em:A.def} and  the orthogonality of the basis functions for scalars yields the relation
%
\begin{equation}
\label{wm:const.pi}
	\tilde{\pi}_{lmk} = -\frac1k j^{(0)}_{lmk} - A_{lmk} 
	-\sum\limits_{k'} \frac{B^{(l)}_{kk'}}{\alpha R kk'} \tilde{A}_{lmk'}	
\end{equation}
%
with the matrix
%
Integrating by parts and using the boundary condition \eqref{appexp:Bessel.bc}, one easily finds that 
%
\begin{equation}
\label{em:Bmat.prop1}
	B^{(l)}_{kk'} = -\frac32 \delta_{kk'} + B^{(l)}_{[kk']}~,
\end{equation}
%
where the brackets around the indices denote anti-symmetrization. Similarly, consider the integral 
%
\[ \tilde{B}^{(l)}_{kk'} = \frac1{c^{(0)}_{lk}c^{(0)}_{lk'}} 
	\int\limits_0^R \rmd r\, r^4 [\partial_r j_l(kr)][\partial_r j_l(k'r)]~, \]
%
which is symmetric in $(k,k')$. Integrate by parts and use the differential equation for spherical Bessel functions to substitute the second derivative, to obtain
%
\begin{equation}
\label{em:Btildemat}
	\tilde{B}^{(l)}_{kk'} = -2B^{(l)}_{k'k} + k^2 C^{(l)}_{kk'} -l(l+1) \delta_{kk'}~, 
\end{equation} 
%
where $C^{(l)}_{kk'}$ is the integral
%
\begin{equation}
\label{em:Cmat.def}
	C^{(l)}_{kk'} = \frac1{c^{(0)}_{lk}c^{(0)}_{lk'}} \int\limits_0^R \rmd r\, r^4 j_l(kr) j_l(k'r)~.
\end{equation}
%
Taking the symmetric and anti-symmetric parts of equation \eqref{em:Btildemat} immediately yields
%
\begin{equation}
\label{em:Bmat.prop2}
	B^{(l)}_{[kk']} = \frac14\left(k'{}^2-k^2\right) C^{(l)}_{kk'}~,
\end{equation}
%
and
%
\begin{equation}
\label{em:Bmat.prop3}
	\tilde{B}^{(l)}_{kk'} = \left[3-l(l+1)\right] \delta_{kk'} +\frac12\left(k'{}^2+k^2\right) C^{(l)}_{kk'}~,
\end{equation}
%
respectively.

